Fast-Slow Recurrent Neural Networks

Processing sequential data of variable length is a major challenge in a wide range of applications, such as speech recognition, language modeling, generative image modeling and machine translation. Here, we address this challenge by proposing a novel recurrent neural network (RNN) architecture, the Fast-Slow RNN (FS-RNN). The FS-RNN incorporates the strengths of both multiscale RNNs and deep transition RNNs as it processes sequential data on different timescales and learns complex transition functions from one time step to the next. We evaluate the FS-RNN on two character level language modeling data sets, Penn Treebank and Hutter Prize Wikipedia, where we improve state of the art results to $1.19$ and $1.25$ bits-per-character (BPC), respectively. In addition, an ensemble of two FS-RNNs achieves $1.20$ BPC on Hutter Prize Wikipedia outperforming the best known compression algorithm with respect to the BPC measure. We also present an empirical investigation of the learning and network dynamics of the FS-RNN, which explains the improved performance compared to other RNN architectures. Our approach is general as any kind of RNN cell is a possible building block for the FS-RNN architecture, and thus can be flexibly applied to different tasks.

==> apendix.tex <==
a
Run the wikipedia page of irrational numbers and start a latex math expression (only 250K character as latex math in enwik8 train set)

Last paragraph of given input: 
\begin{verbatim}
== The square root of 2 ==

One proof of the irrationality of the square root of 2 is the following [[reductio ad absurdum]].    The proposition is proved by assuming the negation and showing that that leads to a contradiction, which means that the proposition must be true.

# Assume that &amp;radic;&lt;font style=&quot;text-decoration: overline&quot;&gt;2&lt;/font&gt; is a rational number. This would mean that there exist integers ''a'' and ''b'' such that ''a'' / ''b'' = &amp;radic;&lt;font style=&quot;text-decoration: overline&quot;&gt;2&lt;/font&gt;.
# Then &amp;radic;&lt;font style=&quot;text-decoration: overline&quot;&gt;2&lt;/font&gt; can be written as an [[irreducible fraction]] (the fraction is shortened as much as possible) ''a'' / ''b'' such that ''a'' and ''b'' are [[coprime]] integers and (''a'' / ''b'')&lt;sup&gt;2&lt;/sup&gt; = 2.
# It follows that ''a''&lt;sup&gt;2&lt;/sup&gt; / ''b''&lt;sup&gt;2&lt;/sup&gt; = 2 and ''a''&lt;sup&gt;2&lt;/sup&gt; = 2 ''b''&lt;sup&gt;2&lt;/sup&gt;.
# Therefore ''a''&lt;sup&gt;2&lt;/sup&gt; is even because it is equal to 2 ''b''&lt;sup&gt;2&lt;/sup&gt; which is obviously even.
# It follows that ''a'' must be even. (Odd numbers have odd squares and even numbers have even squares.)
# Because ''a'' is even, there exists a ''k'' that fulfills: ''a'' = 2''k''.
# We insert the last equation of (3) in (6): 2''b''&lt;sup&gt;2&lt;/sup&gt; = (2''k'')&lt;sup&gt;2&lt;/sup&gt; is equivalent to 2''b''&lt;sup&gt;2&lt;/sup&gt; = 4''k''&lt;sup&gt;2&lt;/sup&gt; is equivalent to ''b''&lt;sup&gt;2&lt;/sup&gt; = 2''k''&lt;sup&gt;2&lt;/sup&gt;.
# Because 2''k''&lt;sup&gt;2&lt;/sup&gt; is even it follows that ''b''&lt;sup&gt;2&lt;/sup&gt; is also even which means that ''b'' is even because only even numbers have even squares.
# By (5) and (8) ''a'' and ''b'' are both even, which contradicts that ''a'' / ''b'' is irreducible as stated in (2).

Since we have found a contradiction the assumption (1) that &amp;radic;&lt;font style=&quot;text-decoration: overline&quot;&gt;2&lt;/font&gt; is a rational number must be false. The opposite is proven. &amp;radic;&lt;font style=&quot;text-decoration: overline&quot;&gt;2&lt;/font&gt; is irrational.

This proof can be generalized to show that any root of any [[natural number]] is either a natural number or irrational.

<math>
\end{verbatim}

only 250K out of 90M characters in the training data is latex math mode
1.19bpc model, 10 consecutive outputs: \\
$x=1$ \\
$X$ \\
%$\mathbb{B}(A)=\mathbf{Q}\qquad\quad\pmatrix$\
$\mathrm{N}(N)=(n-E)!!$ \\
$\mathrm{E}(n,m)=\mathrm{F}(N),\ \mathbf{n}\mathbf{a}^* - (m \in |\mathbf{k})/\mathrm{E}(n)=, \quad $ \\
$\neg (x^2)^n=1$ \\
%$\langle i, y, n|  \rangle = p(A) \lim_{i n \to a}^{n} n_i \leq n_i \end{matrix}$
${\exp(-A-b\theta):1} =-\mathbf{A}d[n]$ \\
$7^3+1 + 2y^4-3 \cdot 4^{2n-1}\cdots = 16$ \\
%$\sqrt{\pi} = \sum_{k=1}^{\infty}\frac{}{2}m \geq q\ge 0} = {k^k \choose k}$




\begin{verbatim}
==The story of the ''Iliad''==
The ''Iliad'' narrates several weeks of action during the tenth and final year of the [[Trojan War]], concentrating on the wrath of [[Achilles]]. It begins with the dispute between Achilles and [[Agamemnon]], and ends with the funeral rites of [[Hector]]. Neither the background and early years of the war ([[Paris (mythology)|Paris]]' abduction of [[Helen]] from [[monarch|King]] [[Menelaus]]), nor its end (the death of [[Achilles]]), are directly narrated in the ''Iliad''.  The ''Iliad'' and the ''Odyssey'' are part of a [[Trojan War cycle|larger cycle of epic poems]] of varying lengths and authors; only fragments survive of the other poems, however.  

Of the many themes in the ''Iliad'', perhaps the most important is the idea of what a hero is. Achilles is forced to make a choice between living a long life or ----

\end{verbatim}

continuation1:
\begin{verbatim}
two without cutting out him more during the month process. His folds sometimes involve the slain and fish, humanoid horizon, and the legs. In many contexts, one should interpret the blessing of Hera to be St Omnu, the first [[Ataris|historical atlas]] finding to him for five years, but to discuss the sources. In his poem ''[[Metamorphoses]]'', Suetonius gathers his harrow with a musglade heart that slows down. 

The shadow of Odysseus hinges like a great angel with a fictionally canisterious [[true sky]], with creatures suchly displayed with his apparellesses and big capes. It was later seen replaced with various children's stories and myths.
\end{verbatim}
continuation2:
\begin{verbatim}
    long ago into a world, like Hellenistic myth and archaeology, known only for his refining of the divine intentions \xe2\x80\x94 some kings of unknown, [[epoch]]e and [[dome]] -- and as well as their genius; thus, they are no longer completely harnessed, as have been thought to be, but coexistent from Athens. Also some of his colleagues are in the study of opposition, but his great association with [[Plato]] does not include them (Plato's ''[[Odyssey]]''). In the apostle's life, Heracles had chosen who might have been entombed in the horse and women.

As ''[[The One Treasure]]'' (found in the ''Iliad'' III, 2) he had teeth, mercenary and vine piercings  to destroy these customs and discovers the raising of a [[passionate burial]] by gold and gold. Hence, as late as 338 B.C., his rostocks were laid out for peacetime in [[Greece]], often for immediacy and at home.
\end{verbatim}
continuation3:
\begin{verbatim}
    an escape from his place, and divides his privilege into a certain fusion of war.  It is simple whether the existence of both the image and Parthenon does not derive from famous authors, occasionally claimed by many scholars to be the end of the [[Priestly Doctrine]].  As ''De Censor, Eccentristibus'' (The History in Republic, Philo: II), written in the Sumerian look, he knows itself but the Leucippus was both &quot;sanctitious&quot; and rebellionable. The two characters subsequently produced a comprehensive lens of versepassages written here.

On the occasion of the [[Fourth Crusade]], Constantine was the longest-serving of the troops hunting. Otherwise, he bore the belts of bones for prayer, paid money to Pope Gregory XII, to bury the bishops contemplating upon his bread and wine. 
\end{verbatim}




==> todo.tex <==
\section{To Dos}
\begin{itemize}
    \item check all the numbers (BPC) wether they are correctly rounded
    \item check consistence, capital letter at Fast cell, Fast layer
    \item Check experiment tables
    \item appendix
    \item new plots 20 epochs of training
\end{itemize}
